On the effect of isotropic and anisotropic dissipative response functions with associated and non-associated flow on the inelastic behaviour of polymeric composites

This article investigates the effect of using isotropic and anisotropic plastic response functions in the analysis of the elastic-plastic response of unidirectional fibre composites on the meso-scale. Three model problems that use a Drucker-Prager-type pressure-dependent yield function are considered to simulate the non-linearities exhibited by a composite material. A further core ingredient is the analysis of a canonical and non-conventional constitutive structure, with respect to associated and non-associated flow response, where the use of latter is motivated by the physical inconsistencies induced by the former under shear dominated loads. These models are evaluated quantitatively by comparison to experimental data.

==> examples/calibration-results/fig.tex <==
\begin{figure}%
\centering%
\small%
%
\includegraphics*[width = \textwidth]{main.eps}
%
\caption{{\bf Calibration results.}
  Comparison of the experimental data \cite{vogler+kyriakides1999} and
  the three meso models responses for (a)~in-plane shear and
  (b)~transverse compression load.}
%
\label{\LABEL}%
\end{figure}%


==> examples/compression-preload-A/fig.tex <==
\begin{figure}%
  \centering  
  %
  \includegraphics*[width = \textwidth]{main.eps}
  %
  \caption{{\bf Predictions for biaxial loads.} Comparison of the
    experimental and associative model responses for the
    $-\sigma_{22}\rightarrow\gamma_{12}$ loading path.}
  \label{\LABEL}%
\end{figure}%


==> examples/compression-preload-NA/fig.tex <==
\begin{figure}%
  \centering  
  %
  \includegraphics*[width = \textwidth]{main.eps}
  %
  \caption{{\bf Predictions for biaxial loads.} Comparison of the
    experimental and non-associative model responses for the
    $-\sigma_{22}\rightarrow\gamma_{12}$ loading path.}
  \label{\LABEL}%
\end{figure}%


==> examples/inconsistencies-corrections/fig.tex <==
\begin{figure}%
  \centering  
  %
  \includegraphics*[width = \textwidth]{main.eps}
  %
  \caption{{\bf Predictions for biaxial loads.} Erroneous predictions
    of the associated flow response and corrected response by the
    non-associative flow rule for shear dominated loads.}
  \label{\LABEL}%
\end{figure}%


==> examples/shear-preload-A/fig.tex <==
\begin{figure}%
  \centering  
  %
  \includegraphics*[width = \textwidth]{main.eps}
  %
  \caption{{\bf Predictions for biaxial loads.} Comparison of the
    experimental and associative model responses for the
    $\tau_{12}\rightarrow-\varepsilon_{22}$ loading path.}
  \label{\LABEL}%
\end{figure}%


==> examples/shear-preload-NA/fig.tex <==
\begin{figure}%
  \centering  
  %
  \includegraphics*[width = \textwidth]{main.eps}
  %
  \caption{{\bf Predictions for biaxial loads.} Comparison of the
    experimental and non-associative model responses for the
    $\tau_{12}\rightarrow-\varepsilon_{22}$ loading path.}
  \label{\LABEL}%
\end{figure}%


==> tables/tab-material-parameters-2.tex <==
\begin{table}[t!]
  \begin{minipage}{\textwidth}
  \caption{Material parameters for Model-II.}
  \label{Table-2}
  \begin{tabular}{cllcll}
    No. & Name                                       & Par.            &        Value       & Unit \\\hline\hline
    1.  & Longitudinal Young's modulus           & $\EMODULUS_1$   & 130000                & $\mathrm{[MPa]}$ \\
    2.  & Transverse Young's modulus             & $\EMODULUS_2$   & 11000                 & $\mathrm{[MPa]}$ \\
    3.  & Longitudinal shear modulus             & $\GMODULUS_{12}$ & 5800                  & $\mathrm{[MPa]}$ \\
    4.  & Transverse shear modulus               & $\GMODULUS_{23}$ & 3720                  & $\mathrm{[MPa]}$ \\
    5.  & Poisson's ratio                        & $\POISSON_{12}$  & 0.306                 & $\mathrm{[-]}$   \\
    6.  & Anisotropic space yield strength       & $Y_{11}$         & $\approx\infty$       & $\mathrm{[MPa]}$ \\
    7.  & Anisotropic space yield strength       & $Y_{22}$         & 158.6                 & $\mathrm{[MPa]}$ \\
    8.  & Isotropic space yield strength         & $\bar{Y}$       & 158.6                 & $\mathrm{[MPa]}$ \\
    9.  & Coefficient of hydrostatic pressure    & $\kappa$        & $1.931\footnote{\textrm{Associative flow}}/1.917\footnote{\textrm{Non-associative flow}}$ & $\mathrm{[-]}$ \\
    10. & Initial yield stress                   & $y_0$           & 20.5                 & $\mathrm{[MPa]}$ \\
    11. & Hardening modulus                      & $h$             & 415.7                & $\mathrm{[MPa]}$ \\
    12. & Pre-strain                             & $\bar\alpha$    & 1$\times$10$^{-12}$   & $\mathrm{[-]}$   \\
    13. & Hardening exponent                     & $n$             & 0.241                & $\mathrm{[-]}$   \\\hline
  \end{tabular}
  \end{minipage}
\end{table}


==> tables/tab-material-parameters-3.tex <==
\begin{table}[t!]
  \begin{minipage}{\textwidth}
    \caption{Material parameters for Model-III}
    \label{Table-3}
    \begin{tabular}{cllcll}
      No. & Name                                   & Par.             & Value   & Unit \\\hline\hline
      1.  & Longitudinal Young's modulus           & $\EMODULUS_1$   & 130000             & $\mathrm{[MPa]}$ \\
      2.  & Transverse Young's modulus             & $\EMODULUS_2$   & 11000              & $\mathrm{[MPa]}$ \\
      3.  & Longitudinal shear modulus             & $\GMODULUS_{12}$ & 5800               & $\mathrm{[MPa]}$ \\
      4.  & Transverse shear modulus               & $\GMODULUS_{23}$ & 3720               & $\mathrm{[MPa]}$ \\
      5.  & Poisson's ratio                        & $\POISSON_{12}$  & 0.306              & $\mathrm{[-]}$   \\
      6.  & Transverse compressive yield stress    & $y_{22c}$        & $24.6\footnote{\textrm{Associative flow}}/27.4\footnote{\textrm{Non-associative flow}}$ & $\mathrm{[MPa]}$ \\[1mm]
      7.  & In-plane shear yield stress            & $y_{12}$         & 9.41               & $\mathrm{[MPa]}$ \\
      8.  & Transverse shear yield stress          & $y_{23}$         & 10.66              & $\mathrm{[MPa]}$ \\
      9.  & Hardening modulus                      & $h$             & 177.5              & $\mathrm{[MPa]}$ \\
      10. & Pre-strain                             & $\bar\alpha$    & 1$\times$10$^{-12}$ & $\mathrm{[-]}$   \\
      11. & Hardening exponent                     & $n$             & 0.246              & $\mathrm{[-]}$   \\\hline
    \end{tabular}
  \end{minipage}
\end{table}

